SpyHammer: Understanding and Exploiting RowHammer under Fine-Grained Temperature Variations

RowHammer is a DRAM vulnerability that can cause bit errors in a victim DRAM row solely by accessing its neighboring DRAM rows at a high-enough rate. Recent studies demonstrate that new DRAM devices are becoming increasingly vulnerable to RowHammer, and many works demonstrate system-level attacks for privilege escalation or information leakage. In this work, we perform the first rigorous fine-grained characterization and analysis of the correlation between RowHammer and temperature. We show that RowHammer is very sensitive to temperature variations, even if the variations are very small (e.g., $\pm 1$ {\deg}C). We leverage two key observations from our analysis to spy on DRAM temperature: 1) RowHammer-induced bit error rate consistently increases (or decreases) as the temperature increases, and 2) some DRAM cells that are vulnerable to RowHammer exhibit bit errors only at a particular temperature. Based on these observations, we propose a new RowHammer attack, called SpyHammer, that spies on the temperature of DRAM on critical systems such as industrial production lines, vehicles, and medical systems. SpyHammer is the first practical attack that can spy on DRAM temperature. Our evaluation in a controlled environment shows that SpyHammer can infer the temperature of the victim DRAM modules with an error of less than $\pm 2.5$ {\deg}C at the 90th percentile of all tested temperatures, for 12 real DRAM modules (120 DRAM chips) from four main manufacturers.

==> biography.tex <==
%%
%% If your work has an appendix, this is the place to put it.
%\newpage
% if you will not have a photo at all:
\newpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/lois_orosa.jpeg}}]{Lois Orosa}
%\begin{IEEEbiographynophoto}{Lois Orosa}
 is the Director of the Galicia Supercomputing Center (CESGA). Previously, he was a senior researcher at SAFARI Research group @ ETH Zürich, Switzerland. He received his PhD degree from the University of Santiago de Compostela, Spain, in 2013. His current research interests are in computer architecture, hardware security, reliability, memory systems, machine learning (ML) accelerators and quantum computing. For more information,
please see his webpage at \url{https://loisorosa.github.io/}
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/ulrich.png}}]{Ulrich Rührmair}
holds a PhD in computer science from TU Berlin, a PhD in electrical engineering from TU Munich, and an MSc in mathematics from Oxford University. He is a research professor at the University of Connecticut and currently also a guest professor at LMU Munich. His research interests include applied cryptography and computer security in general, as well as Physical Unclonable Functions (PUFs) and related physical security primitives in particular. He is the founder and current steering committee chair of the ASHES workshop, an annual workshop at ACM CCS since 2017. Furthermore, he is an associate editor at the IEEE Transactions on Information Forensics and Security, Journal of Cryptographic Engineering, Journal on Hardware and Systems Security, and EURASIP Journal on Information Security. Since 2022, he is also a co-speaker of the research focus on “Physics and Security” at the Center for Advanced Studies at LMU Munich.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/giray.png}}]{A. Giray Ya\u{g}l{\i}k\c{c}{\i}}
is a Ph.D. candidate in the Safari Research Group at ETH Zürich, working with Prof. Onur Mutlu. His current broader research interests are computer architecture, systems, and hardware security, focusing on DRAM robustness and performance. In particular, his Ph.D. research focuses on understanding and solving the RowHammer vulnerability, on which he has several publications. Giray received his B.S. degree in Electrical Engineering and M.Sc. degree in Computer Engineering from TOBB University of Economics and Technology, Ankara, Turkiye and he holds a second M.Sc. in Computer Science from University of Notre Dame, IN, USA. Giray holds an honorable mention from the Intel Hardware Security Academic Award, 2021, and is the First-Place winner in the graduate category of Student Research Competition in PACT, 2023. Giray’s research is partly supported by Google and the Microsoft Swiss Joint Research Center.
\end{IEEEbiography}
%\
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/haocong.png}}]{Haocong Luo}
is a Ph.D. student in the Safari Research Group at ETH Zürich, advised by Prof. Onur Mutlu. His current research interests are in computer architecture, focusing on memory systems and DRAM. Haocong received his B. Eng. degree in Computer Science from ShanghaiTech University, and his M.Sc. degree in Computer Science from ETH Zürich.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/ataberk.png}}]{Ataberk Olgun}
is a Ph.D. student at ETH Zürich. He received his master’s degree in Computer Engineering from TOBB University of Economics and Technology. His research interests include memory system reliability, safety, and performance. For more information, please see his webpage at \url{https://aolgun.com}.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/patrick.png}}] {Patrick Jattke} is a doctoral student at ETH Zürich, Switzerland. His main research interests are in the area of memory disturbance errors, specifically Rowhammer. Prior to his current position, Patrick received his B.Sc. from TU Darmstadt, Germany, in Computer Science and M.Sc. in IT Systems Engineering from HPI Potsdam, Germany.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/minesh.png}}]{Minesh Patel}
received his Ph.D. from ETH Zürich and dual B.S. degrees from UT Austin in physics and electrical engineering. His doctoral thesis focuses on overcoming performance, reliability, and security challenges in the memory system. In particular, his dissertation identifies and addresses new challenges for system-level error detection and mitigation targeting memory chips with integrated error correcting codes (ECC). He also worked collaboratively on understanding and solving the RowHammer vulnerability, near-data processing, efficient virtual memory management, and new hardware security primitives. Minesh’s graduate work has been recognized with several honors, including DSN’19 and MICRO’20 Best Paper Awards, the William Carter Dissertation Award in Dependability, the ETH Doctoral Medal, and induction into the ISCA Hall of Fame.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/jeremie.png}}]{Jeremie S. Kim}
 earned his Ph.D. in Electrical and Computer Engineering from Carnegie Mellon University in August 2020. His thesis won the 2020 EDAA Outstanding Dissertation Award in the area of “new directions in safety, reliability and security-aware hardware design, validation and test for systems and circuits.” His current research interests are in computer architecture, memory latency/power/reliability, hardware security, and bioinformatics, and he has several publications on these topics. Previously, Jeremie received the BS and MS degrees in Electrical and Computer Engineering from Carnegie Mellon University in Pittsburgh, Pennsylvania, in 2015.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/kaveh.png}}]{Kaveh Razavi}
 is an assistant professor at ETH Zurich where he leads 
the Computer Security Group. His research interests are in the area of 
systems and security. More recently, he has been involved in the 
discovery and exploitation of many high-profile hardware vulnerabilities 
in commodity hardware components such as DRAM and CPU. These efforts 
have won him and his collaborators many awards, including best paper 
awards at IEEE S\&P and MICRO, and five Pwnies at BlackHat.
\end{IEEEbiography}
%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Pictures/Onur.jpeg}}]{Onur Mutlu}
%\begin{IEEEbiographynophoto}{Onur Mutlu}
is a Professor of Computer Science at ETH Zurich. He is
also a faculty member at Carnegie Mellon University, where he
previously held the Strecker Early Career Professorship.  His 
research interests are in computer architecture, systems,
hardware security, bioinformatics. A variety of techniques he,
along with his group and collaborators, has invented over the years
have influenced industry and are employed in commercial
microprocessors and memory/storage systems. He started the Computer Architecture Group at Microsoft Research (2006-2009), and held various product and research positions
at Intel Corporation, AMD, VMware, and Google.  He is an ACM Fellow, IEEE Fellow, and an elected member of the Academy of Europe. His computer architecture and digital design course lectures are freely available (\url{https://www.youtube.com/OnurMutluLectures}). His research group
makes a wide variety of software and hardware artifacts freely
available online (\url{https://safari.ethz.ch/}). 
\end{IEEEbiography}

==> sections/03_threat_model.tex <==
\section{Threat Models}
%We build two variants of the \mechanism{} attack that have two different threat models.

We assume two different threat models for 1)~spying on relative temperature changes and 2)~spying on absolute temperature changes.

% Threat Model
\subsection{Spying on Relative Temperature Changes.}
\label{sec:threatmodel1}
We assume an attacker with \emph{no} prior knowledge or physical access to the victim DRAM module. Thus, the victim's software and hardware can not be characterized or modified by the attacker prior to the attack. 

With the goal of building models that correlate \gls{ber} with temperature, the attacker can purchase many DRAM modules from different manufacturers and has the infrastructure to control the DRAM temperature of those modules in a fine-grained manner.

\subsection{Spying on Absolute Temperature Changes.}
\label{sec:threatmodel2}
We assume an attacker that has access to the victim DRAM module before performing the attack, and they can characterize the bit errors caused by RowHammer in a controlled environment at different temperatures.



==> sections/06_absolute_spyHammer.tex <==
\section{Spying on Absolute Temperature Values with SPYHAMMER}
\label{sec:varianttwo}

This variant of the \mechanism{} attack aims to spy on absolute values of temperature. \agy{To do} so, the attacker must characterize the victim DRAM module prior to the attack (see Section~\ref{sec:threatmodel2}) under different temperature conditions. Thus, the attacker does not need to reverse engineer the model of the victim DRAM module, as in Section~\ref{sec:identify_victim}. Because the attacker uses the victim DRAM module to build the polynomial regression model, the temperature estimations are absolute and more accurate, as we demonstrate in Section~\ref{sec:evaluation_ber}. The rest of the attack remains the same as in Section~\ref{sec:variantone}.

We discuss the limitations of this attack model in Section~\ref{sec:limitations}.

%\subsection{Threat Model}
\vspace{0.2cm}
\noindent{\bf Threat Model.}
\label{sec:threatmodel2}
We assume an attacker that has access to the victim DRAM module before performing the attack, and they can characterize the bit errors caused by RowHammer in a controlled environment at different temperatures.

%\loiscomment{Explain the methodology in the evaluation}

% % Threat MOdel
% \subsection{Threat Model}
% \label{sec:threatmodel2}

% For measuring absolute temperatures using \mechanism{}, we need to assume a different thread model than for measuring relative temperature changes (Section~\ref{sec:variantone}).

% We assume an attacker that has physical access to the victim DRAM device before production. The attacker can induce bitflips in the victim DRAM row under a wide variety of temperatures by using the methodology in Section~\ref{sec:methodology}.


% Detecting the DRAM module
%\subsection{Pre-attack: Characterizing the Victim DRAM module}
%\label{sec:preliminaries2}

%\loiscomment{Preliminaries from variant 1 + characterize the victim DRAM module}
%\loiscomment{We need to characterize just to Make relative numbers become absolute numbers. For doing so, we just need to characterize a few temperature points, and detect a cell that flips only at one specific temperature point. Probably we need several points}

%To perform the \mechanism{} attack on absolute temperature values, the attacker needs to characterize the \gls{ber} and the spot cells of the victim DRAM module. With this information, they can build a precise polynomial regression model, and perfectly map spot cells to DRAM temperature.  % For doing that, the attacker can use the infrastructure described in Section~\ref{sec:methodology}.


% Discussion
% \subsection{Discussion}
% \label{sec:discussion2}
% \loiscomment{discuss limitations}





==> sections/08_evaluation.tex <==
% DRAM Characterization
\section{Evaluation}
\label{sec:evaluation1}

We evaluate the \mechanism{} accuracy and sensitivities when using both \gls{ber} (Section~\ref{sec:evaluation_ber}) and canary cells (Section~\ref{sec:canary_cell_analysis}) to spy on relative temperature changes and absolute temperature.

%%%%%%%%%%%%%%%%%
% BER Analysis
%%%%%%%%%%%%%%%%%
\subsection{BER Characterization and Analysis}
\label{sec:evaluation_ber}

We characterize and analyze the correlation between \gls{ber} and temperature for four different manufacturers. Figure~\ref{fig:tempBER} shows the RowHammer-induced \gls{ber} for temperatures from $50^\circ$C to $95^\circ$C. We analyze 12 DRAM modules, 3 identical modules (i.e., manufacturing data, technology node, chip identifier, etc.) for each  DRAM manufacturer. We use a memory region of 192MB (i.e., 24K DRAM rows) for each DRAM module, and we repeat each experiment 20 times for each temperature point. We plot a line for each module (in the same color as the points in the plot) that represents the polynomial regression model we use for each module.

\begin{figure}[h] \centering
    \includegraphics[width=1.0\linewidth]{Results/ber_spyhammer2-crop.pdf}
    \caption{Correlation between RowHammer-induced bitflips per row (\gls{ber}) and temperature.} 
    \label{fig:tempBER}
\end{figure}

We make five observations. 
%
First, the absolute \gls{ber} values of 2 identical modules from the same manufacturer can differ significantly. For example, Module Id. 3 from Mfr. A shows in the order of 2.5$\times$ more bitflips than Module Id. 2. 
%
Second, the form of the curve for a particular DRAM module is similar to the curve from other modules from the same manufacturer. For example, although absolute \gls{ber} values differ slightly, all curves from Mfr. D modules have approximately the same shape.
%
Third, the \gls{ber} can increase (e.g., Mfr. A) or decrease (e.g., Mfr. B) depending on the DRAM manufacturer. 
%
Fourth, most modules (i.e., Mfrs. A, B, and D) show a linear relation between \gls{ber} and temperature. In Mfr. C, we observe that the relation is not linear if the temperature is higher than \SI{70}{\celsius}. 
%
Fifth, the \gls{ber} across the 20 repetitions of the experiment is very similar, as there is little variation within the y-axis for each temperature point.

We conclude that the similar correlation between \gls{ber} and temperature within the same manufacturer can be used to estimate the victim temperature.\footnote{For a particular model of a Mfr. D module (not shown in our evaluation results), we can not observe enough RowHammer-induced bitflips to make conclusive observations about the relation RowHammer/Temperature.} 
%
%
To do so, we find that a polynomial regression model of order 3 is good enough to accurately model the correlation beetween \gls{ber} an temperature for all modules we test. Table~\ref{tab:linear_regresion} shows the polynomial regression equations inferred for each DRAM module. %The polynomial regression equation has the format $y = Ax + B$, where $x$ is the temperature, $y$ is the \gls{ber}, $A$ is the constant that defines the slope of the line, and $B$ is the point where the line crosses the y-axis (i.e., the \gls{ber} at \SI{0}{\celsius}).

\begin{table}[h]
 \scriptsize\setlength{\tabcolsep}{2pt}
  \begin{center}
  \begin{tabular}{c|l} 
  \toprule
  {\bf Id.}  & {\bf Polynomial Regression}\\
  \midrule
  %1 & A &  y = 0.0185x + 0.9921\\
  1 &   $y = -(1.9*10^{-6})*x^3 + (4.8*10^{-4})*x^2 - (2.2*10^{-2})*x + 2.1 $\\
  %2 &   y = 0.0139x + 0.5876\\
  2 &   $y = +(6.8*10^{-7})*x^3 - (6.4*10^{-5})*x^2 + (1.2*10^{-2})*x + 0.8$ \\
  3 &   $y = +(4.0*10^{-7})*x^3 +(3.0*10^{-5})*x^2  + (2.0*10^{-2})*x + 2.3$ \\
  \midrule
  %3 &   y = -0.698x + 194.7173\\
  4 &   $y = - (1.9*10^{-4})*x^3 + (4.0*10^{-2})*x^2 - 3.5*x +260$\\
  %4 &   y = -0.8067x + 198.0824\\
  5 &   $y = +(9.5*10^{-5})*x^3 - (2.1*10^{-2})*x^2 + 0.8*x +157.7$ \\
  6 & $y =  +(2.4*10^{-4})*x^3 -(4.9*10^{-2})*x^2 + (2.5)*x + 121.8$ \\
  \midrule
  %5 &   y = 2.0515x + 72.5439\\
  7 &   $y = + (1.4*10^{-3})*x^3 -0.2*x^2 + 15.6*x -152.2 $\\
  %6 &   y = 0.7682x + 157.1299\\
  8 &   $y = +(5.1*10^{-3})*x^3 -1.0*x^2 +64.1*x -1201.8 $\\
  9 &   $y = +(8.1*10^{-5})*x^3 - (9.9*10^{-3})*x^2 + (0.9)*x + 167.6$\\
  \midrule
  %7 &   y = (5.4879x + 70.6327)/1000 \\
  10 &   $y = +(4.5*10^{-7})*x^3 - (6.3*10^{-5})*x^2 + (7.4*10^{-3})*x + 0.1$ \\
  %8 &   y = (4.8541x + 95.5300)/1000 \\
  11 &   $y =  +(3.4*10^{-7})*x^3 - (4.3*10^{-5})*x^2 + (5.7*10^{-3})*x + 0.1$\\ 
  12 &   $y = - (1.2*10^{-7})*x^3 + (6.4*10^{-5})*x^2 + (2.5*10^{-3})*x + 0.3) $\\
\bottomrule
\end{tabular}
\caption{Polynomial regression that models the correlation between \gls{ber} and temperature.}
\label{tab:linear_regresion}
\end{center}
\end{table}


We observe that the regression curve is reasonably similar between modules from the same manufacturers. We conclude that we can spy on temperature by using a polynomial regression model from a DRAM module that is the same model as the victim DRAM module. However, we assume that the accuracy of the model can significantly change depending on the DRAM module and the threat model.

\vspace{0.2cm}
\noindent{\bf Methodology for Measuring Accuracy.} To evaluate the accuracy of the polynomial regression model to estimate temperature, we select a sequence of 720 random temperature points in the tested range (i.e., from \SI{50}{\celsius} to \SI{95}{\celsius}), and we measure the accuracy of the estimation for all temperatures in the sequence. For spying on relative temperature changes, we use the change between consecutive temperature points in the sequence, and for spying on absolute temperature, we use each temperature point in the sequence. We make sure that the sequence of random temperatures includes extreme temperature changes (e.g., from \SI{95}{\celsius} to \SI{50}{\celsius}), and small temperature changes (e.g., from \SI{50}{\celsius} to \SI{51}{\celsius}).




% \vspace{0.2cm}
% \noindent{\bf Methodology for Evaluating Accuracy.}
% To evaluate the accuracy of the polynomial regression model for spying on relative temperature changes, we use the following methodology: \loiscomment{This should be in the evaluation}
% \begin{enumerate}
%     \item Using a DRAM module that is the same model as the victim DRAM module, the attacker builds a polynomial regression  model  by  capturing  the \gls{ber} for  all  temperatures from \SI{50}{\celsius}  to \SI{95}{\celsius},  in  temperature  steps  of \SI{1}{\celsius}.  We construct the model by using 20 \gls{ber} measurements per temperature point (see Section~\ref{sec:methodology}).
%     \item To evaluate the accuracy of the attack, we generate a sequence of random temperature points within the tested temperature range, so we make sure we evaluate both small and large temperature changes. 
%     \item We use a polynomial regression model to infer the temperature of the victim DRAM module. As the absolute values might differ significantly, we can rely only on the relative temperature changes (the curve of the polynomial regression is similar across modules from the same manufacturer).
%     \item We  calculate  the  error  between  the  delta  temperature variation  predicted  by  the  polynomial  regression  model,  and the real delta temperature variation of the victim DRAM chip.
% \end{enumerate}

\vspace{0.2cm}
\noindent{\bf Accuracy when Spying on Relative Temperature Changes.} We study the accuracy of spying the relative temperature changes of the victim DRAM module using a polynomial regression model obtained from a DRAM module that is the same model as the victim DRAM module. Figure~\ref{fig:relative_temperatureResolution} shows the probability distribution of the temperature error when we use the polynomial regression model. For each victim DRAM module of each manufacturer, we use a polynomial regression model obtained from one of the other two modules we test from the same manufacturer. Table~\ref{tab:percentile_relative} shows the maximum error in the estimation of the relative temperature changes (in \SI{}{\celsius}), for $90^{\mathrm{th}}$ percentile of the error distribution. We show values for temperature changes up to \SI{45}{\celsius} (L), and for temperature changes up to \SI{5}{\celsius} (S), which should be the common case if the \gls{ber} monitoring frequency is large enough.

\begin{figure}[h] \centering
    \includegraphics[width=1.0\linewidth]{Results/relativeErrorBER2-crop.pdf}
\caption{Error of the relative temperature change estimation obtained using a polynomial regression model from a DRAM module that is the same model as the victim DRAM module.}
    \label{fig:relative_temperatureResolution}
\end{figure}

\begin{table}[h]
 %\scriptsize
 \setlength{\tabcolsep}{2pt}
  \begin{center}
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c} 
  \toprule
  {\bf Module Id.} & {\bf 1} & {\bf 2} & {\bf 3} & {\bf 4} & {\bf 5} & {\bf 6} & {\bf 7} & {\bf 8} & {\bf 9} & {\bf 10} & {\bf 11} & {\bf 12}\\
    \midrule
  {\bf Error (L)$^\dagger{}$ (\SI{}{\celsius})} & 7.8 & 12.6 & 5.6 & 3.9 & 4.6 & 3.9 & 14.5 & 6.6 & 23.1 & 2.0 & 1.9 & 1.0 \\
  {\bf Error (S)$^\ddagger{}$ (\SI{}{\celsius})} & 3.1 & 3.1 & 3.3 & 3.4 & 2.4 & 3.2 & 2.6 & 3.3 & 2.6 & 2.0 & 1.9 & 1.0\\
\bottomrule
\end{tabular}
    \begin{flushleft}
       \centering{$^\dagger{}$} for relative temperature changes up to \SI{45}{\celsius}.\\
       \centering{$^\ddagger{}$} for relative temperature changes up to \SI{5}{\celsius}
    \end{flushleft}  
\caption{Maximum temperature error (in \SI{}{\celsius}) for $90^{\mathrm{th}}$ percentile of the error distribution, when estimating relative temperature changes.}
\label{tab:percentile_relative}
\end{center}
\end{table}

We make two observations. First, the error of the temperature estimated by the regression model is reasonably low for modules from Mfr. B (Module Id. 4, 5, 6) and Mfr. D (Module Id. 10, 11, 12), because the correlation between \gls{ber} and temperature is very similar across all modules from the same manufacturer. We find that the error is larger for Mfr. A (Module Id. 1, 2, 3) and Mfr. C (Module Id. 7, 8, 9) because in each of these manufacturers, there is one module that has a slightly different curve than the other two modules. Second, in many cases, the estimation error is zero (i.e., error = \SI{0}{\celsius}). We observe that when the temperature change is small (e.g., $<$\SI{5}{\celsius}), the estimation error is small for all modules ($<$\SI{3.5}{\celsius}), whereas when the temperature change is large (e.g., up to \SI{45}{\celsius}) the estimation error is much larger (only 3 modules have less than \SI{3.5}{\celsius} error). 

We make two conclusions. First, for all possible temperature changes (i.e., from very small to very large temperature changes), a polynomial regression model works well if the modules show very similar correlations between \gls{ber} and temperature. Second, for small temperature changes, we can get accurate temperature estimations from all modules we test. By sampling with enough frequency, this should be always the case in regular conditions. 

\vspace{0.2cm}
\noindent{\bf Accuracy when Spying on Absolute Temperature Values.} We study the accuracy of spying the absolute temperature of the victim DRAM module using a polynomial regression model obtained from the victim DRAM module itself. Figure~\ref{fig:absolute_temperatureResolution} shows the probability distribution of the error when estimating the absolute temperature. Table~\ref{tab:percentile_absolute} shows the maximum error in the estimation of the absolute temperatures (in \SI{}{\celsius}), for $90^{\mathrm{th}}$ percentile of the error distribution.


\begin{figure}[h] \centering
    \includegraphics[width=1.0\linewidth]{Results/absoluteErrorBER2-crop.pdf}
    \caption{Absolute temperature error estimated for the victim DRAM module with a polynomial regression model obtained from the victim DRAM module.} 
    \label{fig:absolute_temperatureResolution}
\end{figure}

\begin{table}[h]
 %\scriptsize
 \setlength{\tabcolsep}{2pt}
  \begin{center}
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c} 
  \toprule
  {\bf Module Id.} & {\bf 1} & {\bf 2} & {\bf 3} & {\bf 4} & {\bf 5} & {\bf 6} & {\bf 7} & {\bf 8} & {\bf 9} & {\bf 10} & {\bf 11} & {\bf 12}\\
    \midrule
  {\bf Error (\SI{}{\celsius})} & 0.5 & 1.2 & 0.5 & 1.4 & 2.3 & 2.3 & 0.9 & 1.7 & 1.9 & 0.5 & 0.6 & 0.5 \\
\bottomrule
\end{tabular}

\caption{Maximum temperature error (in \SI{}{\celsius}) for $90^{\mathrm{th}}$ percentile of the error distribution, when estimating absolute temperatures.}
\label{tab:percentile_absolute}
\end{center}
\end{table}

We make the main observation that the absolute temperature estimations are very accurate for most of the DRAM modules. All modules we tested show an error lower than \SI{2.5}{\celsius} for $90^{\mathrm{th}}$ percentile. We conclude that 1) using a regression model from the same victim DRAM module provides accurate results, and 2) a polynomial regression model is enough to accurately estimate absolute temperatures in most modules.

% Resolution of the BER attack
\vspace{0.2cm}
\noindent{\bf BER Variations in Different DRAM Regions.}
%
To make the attack less intrusive and simple (i.e., reduce the probability of being detected), an attacker can monitor the \gls{ber} in a smaller DRAM region to reduce the number of RowHammer accesses. We study if different DRAM regions within a DRAM module have a similar \gls{ber} behavior. Figure~\ref{fig:BERreg} shows the correlation between the \gls{ber} and the temperature, for 48 different DRAM regions of 4MB, for all DRAM modules we test. %Region 1 corresponds to the first 8K rows, region 2 corresponds to the middle 8k rows, and region 3 corresponds to the last 8k rows of the DRAM module.  %\loiscomment{explain how we choose the regions}%In practice, all DRAM regions of the same module have similar \gls{ber} behavior, so there is no need to know the exact region in which we are performing the attack, nor the memory region allocated by the OS needs to be contiguous.

\begin{figure}[h] \centering
    %\includegraphics[width=1.0\linewidth]{Results/regions_spyhammer-crop.pdf}
    %\includegraphics[width=1.0\linewidth]{Results/regions_boxplot-crop.pdf}
    \includegraphics[width=1.0\linewidth]{Results/regions_boxplot2-crop.pdf}
    \caption{Boxplot of RowHammer-induced \gls{ber} in 48 different 4MB memory regions from the same DRAM module.}
    \label{fig:BERreg}
\end{figure}

We make two observations. First, the correlation of \gls{ber} with temperature follows the same trend for all regions we test (i.e., the curves for different regions within the same module are similar). Second, the variation on absolute \gls{ber} values across different regions is reasonably small for all DRAM modules. %First, for modules from Mfr. A, B and C (i.e, 1,2,3,4,7 and 8), the correlation of \gls{ber} with temperature is very similar for all regions we test. Second, for modules from manufacturer B, there is not a very clear correlation between \gls{ber} and temperature. %Our main observation is that the \gls{ber} 


We conclude that the attacker can use any region in memory to perform the attack, which simplifies the requirements of the attack (i.e., no need for reverse engineering the physical location of the memory region to find an appropriate region). %\loiscomment{write}

%\loiscomment{PLot how it changes the BER in different DRAM regions of the same module}
%\loiscomment{If it is very similar, we dont need to know in which region we are... it is enough with having a continuous memory region}

%\loiscomment{Plot Jaccard Indices between regions}
%%%%%%%%%%%%%%%%

\vspace{0.2cm}
\noindent{\bf Sensitivity to Different Region Sizes.}
To improve performance and reduce the probability of the attack being detected, the attacker can reduce the size of the DRAM region used for performing the attack. Figure~\ref{fig:regionSize} shows the mean error of the temperature change estimated by the polynomial regression model for different region sizes from 512 rows (4MB) to 24k rows (192MB). The color of the bars represents the two threat models we evaluate: 1) spying on relative temperature changes, and 2) spying on absolute temperatures.


\begin{figure}[h] \centering
    %\includegraphics[width=1.0\linewidth]{Figures/tempIntervals-crop.pdf}
    \includegraphics[width=1.0\linewidth]{Results/regionSize_barplot-crop.pdf}
    \caption{Mean error of the temperature estimated by the polynomial regression model for different region sizes.}
    \label{fig:regionSize}
\end{figure}

We make three observations. 
%
First, we can reduce the region size from 24k to 2k with minor or none increase in the mean error for all cases we test. 
%
Second, for region sizes lower than 2k, the mean error increases significantly in many cases. For example, modules from Mfr. B (Module Id. 4, 5 6) show a very significant error increase in the absolute temperature estimation.
%
 Third, the mean error values show similar trends for both relative \agy{and absolute} temperature changes for most modules we test. However, the error increases more quickly when reducing the region size when estimating absolute temperatures. \loiscomment{Why?? reason about it}

We conclude that the attacker can use regions of size as small as 2k rows (i.e., 16MB) for spying on temperature while maintaining reasonable levels of accuracy.

% canary Cell Analysis
\subsection{Canary Cell Analysis}
\label{sec:canary_cell_analysis}
% Resolution of the canary cell attack

Canary cells can be used to reduce to optimize the \mechanism{} attack by reducing the number of hammers required to perform the attack (see Section~\ref{sec:variantone}). We analyze the number of canary cells we observe for each temperature point that can be used to estimate the temperature of the victim DRAM module. Figure~\ref{fig:num_canary_cells} shows the number of canary cells (in logarithmic scale) per temperature point, and the minimum number of canary cells across all temperature points. In the enrollment process, we repeat each experiment 10 times for each temperature point, and we select those cells that experience bitflips at least once.

\begin{figure}[h] \centering
    %\includegraphics[width=1.0\linewidth]{Figures/tempIntervals-crop.pdf}
    \includegraphics[width=1.0\linewidth]{Results/spotCells2-crop.pdf}
    %\caption{Temperature range at which DRAM cells are vulnerable to RowHammer, for particular DRAM module from manufacturer \loiscomment{X}} 
    \caption{Number of canary DRAM cells (i.e., DRAM cells that flip only at one temperature) that flip at each temperature point.}
    \label{fig:num_canary_cells}
\end{figure}

We make two observations. First, all temperature points we test have at least 18 canary cells (Module Id. 11, and 12) in the worst case, in all modules we test. The minimum number of canary cells is large enough, as it only requires one single canary cell to estimate the temperature at a particular temperature point. Second, there are more canary cells on the extremes of the temperature range. This phenomenon is caused by the limited temperature range, so some canary cells at the lower limit (\SI{50}{\celsius}) might not be canary cells anymore if they result to flip also at \SI{49}{\celsius}.

We conclude that all modules we test have a large enough number of canary cells (i.e., more than one) for each temperature point, so they can be used to reliably infer the DRAM temperature.

%\loiscomment{Simplify: We only need a Table with the minimum, maximum, and average}
%\loiscomment{Represent this data better. Do we need to plot all the cells?}
%\loiscomment{What is our target temperature}

\vspace{0.2cm}
\noindent{\bf Canary Cell Accuracy.}
%\subsubsection{Canary Cell Accuracy}
\label{sec:evaluation_canarycell} 
%We identify canary cells by 1) repeating our experiments ten times for each temperature to identify the canary cells, and 2) testing
We measure the accuracy of \mechanism{} when using canary cells.   Figure~\ref{fig:temperatureResolutioncanary} shows the probability distribution of the temperature errors when spying on absolute temperature using canary cells.\footnote{Similarly, canary cells can also be used to estimate relative temperature changes.} We use 10 iterations of our experiments to perform the enrollment process (i.e., identify the canary cells), and another 10 different iterations to monitor the canary cells and spy on temperature. %temperature accuracy we can achieve from the modules we test using canary cells.

\begin{figure}[h] \centering
    \includegraphics[width=1.0\linewidth]{Results/canary_accuracy2-crop.pdf}
    \caption{Probability distribution of the temperature estimation errors using canary cells.}
    \label{fig:temperatureResolutioncanary}
\end{figure}

%\loiscomment{Train with the first 10 repetitions}
%\loiscomment{Get accuracy with the other 10 repetitions}
%\loiscomment{Report if the Canary cell reports the correct temperature}

We make two main observations. First, canary cells can estimate the temperature accurately (i.e., no errors) with more than 25\% probability, with some cases close to 50\% (e.g., Module Id. 4, 8). Second, canary cells can be used to estimate temperature with less than $\pm$\SI{5}{\celsius} error with very high probability. % the probability distribut

We conclude that canary cells can be used to estimate temperature with significant accuracy, while reducing the number of hammers significantly. For example, if an attacker wants to know if the temperature is \SI{60}{\celsius}, it only has to monitor a canary cell that flips only at that temperature point, instead of hammering a large region of memory (see Section~\ref{sec:evaluation_ber}). 

% \subsection{Evaluation in a Real System}
% \loiscomment{Haocong, Kaveh, Patrick}

% To demonstrate that our observations on an FPGA-based testing platform remain valid on a real-world system, we perform \mechanism{} in an unmodified commodity system.

% \subsubsection{Experimental Setup}
% \loiscomment{Include characteristics of the machine and the OS}
% We conduct our experiments on an Intel Core i7-8700K, mounted on an commodity DDR4 mainboard (ASUS ROG STRIX Z390E).
% For the bank/rank addressing functions and the row mask, we rely on reverse-engineering results from previous work~\cite{de_ridder_smash_2021}.
% We use the recently released, open-source Blacksmith RowHammer fuzzer to find access patterns that trigger bitflips~\cite{jattke_blacksmith_2022} on DDR4 DRAM devices with enabled TRR mitigations.
% Like for the FPGA setup (see Section~\ref{subsec:temp_controller}), we apply insulation around the DRAM module and use the same heating and measuring infrastructure.

% \subsubsection{Results}

% \subsection{\mechanism{} Performance Analysis}
% \label{sec:evaluation_performance}

% We evaluate the performance of \mechanism{} using \gls{ber}, canary cells, and different memory region sizes. We compare our mechanism to~\cite{}, which uses cell retention time to infer temperature.

% \loiscomment{This section should include a comparison between BER vs canary cell performance and number of accesses we need}
% \loiscomment{Use performance numbers from Haocong experiments}



==> sections/10_exploitability_analysis.tex <==
\section{Correlation between Exploitability and Temperature}
\label{sec:exploitability_analysis}

\loiscomment{How do we fit this analysis in the paper?}
\loiscomment{Discuss with Kaveh and Patrick}
